Block and Detail: Scaffolding Sketch-to-Image Generation

We introduce a novel sketch-to-image tool that aligns with the iterative refinement process of artists. Our tool lets users sketch blocking strokes to coarsely represent the placement and form of objects and detail strokes to refine their shape and silhouettes. We develop a two-pass algorithm for generating high-fidelity images from such sketches at any point in the iterative process. In the first pass we use a ControlNet to generate an image that strictly follows all the strokes (blocking and detail) and in the second pass we add variation by renoising regions surrounding blocking strokes. We also present a dataset generation scheme that, when used to train a ControlNet architecture, allows regions that do not contain strokes to be interpreted as not-yet-specified regions rather than empty space. We show that this partial-sketch-aware ControlNet can generate coherent elements from partial sketches that only contain a small number of strokes. The high-fidelity images produced by our approach serve as scaffolds that can help the user adjust the shape and proportions of objects or add additional elements to the composition. We demonstrate the effectiveness of our approach with a variety of examples and evaluative comparisons. Quantitatively, evaluative user feedback indicates that novice viewers prefer the quality of images from our algorithm over a baseline Scribble ControlNet for 84% of the pairs and found our images had less distortion in 81% of the pairs.

==> problem_statement.tex <==
\section{Problem Statement}

This is where we need our principles of sketching and how iterative sketching + visualization guides us toward a good final image. 

\begin{enumerate}
    \item Sketch guidance enables user to control contours of generated objects--and control them to the desired degree.
    \item Image generation can help user iterate on sketch to help converge on desired controls
\end{enumerate}

The drawing process has two key modes:
\begin{enumerate}
    \item Blocking: drawing lines that very roughly describe the shape of a desired object when we don't really know how exactly we'd like the contours to turn out. 
    \item Detailing: drawing lines that we want to be adhered to exactly as the edges of objects in the generated images.
\end{enumerate}

\vishnu{Now starting the sketch definition I'm going to carry through to the methods}
We define sketch $S$ as the following:
\begin{enumerate}
    \item A text prompt $p$, describing the image to be generated
    \item \blocking image $b$, a binary image corresponding to \blocking strokes offering loose control over the contours of the generated image
    \item \detail image $b$, a binary image corresponding to \detail strokes offering fine-grained control over the contours of the generated image
\end{enumerate}

Given input sketch $S$, we seek to generate an output image $x^*$ with the following properties:
\begin{enumerate}
    \item Respect the \detail lines precisely
    \item Respect the \blocking lines roughly
    \item Generate complementary content in regions where no lines are drawn
\end{enumerate}

How do we define success? Note that the notion we have in mind of what we'd like to draw can change over time. 

